Effective Human-AI Teams via Learned Natural Language Rules and Onboarding

People are relying on AI agents to assist them with various tasks. The human must know when to rely on the agent, collaborate with the agent, or ignore its suggestions. In this work, we propose to learn rules, grounded in data regions and described in natural language, that illustrate how the human should collaborate with the AI. Our novel region discovery algorithm finds local regions in the data as neighborhoods in an embedding space where prior human behavior should be corrected. Each region is then described using a large language model in an iterative and contrastive procedure. We then teach these rules to the human via an onboarding stage. Through user studies on object detection and question-answering tasks, we show that our method can lead to more accurate human-AI teams. We also evaluate our region discovery and description algorithms separately.

==> sc_bdd.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Screenshots of User Study Interface}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{figure}[h]
    \centering
        \resizebox{\textwidth}{!}{

    \includegraphics{sc_study_bdd/sc1.PNG}
}
    \caption{Consent Form}
\end{figure}

\begin{figure}[h]
\centering
\resizebox{\textwidth}{!}{
\includegraphics{sc_study_bdd/sc2.PNG}
}
\caption{User Information Collection}
\end{figure}

\begin{figure}[h]
\centering
\resizebox{\textwidth}{!}{
\includegraphics{sc_study_bdd/sc3.PNG}
}
\caption{Practice Task instructions}
\end{figure}

\begin{figure}[h]
\centering
\resizebox{\textwidth}{!}{
\includegraphics{sc_study_bdd/sc4.PNG}
}
\caption{Prediction without AI interface}
\end{figure}

\begin{figure}[h]
\centering
\resizebox{\textwidth}{!}{
\includegraphics{sc_study_bdd/sc5.PNG}
}
\caption{Instructions for the onboarding phase}
\end{figure}

\begin{figure}[h]
\centering
\resizebox{\textwidth}{!}{
\includegraphics{sc_study_bdd/sc6.PNG}
}
\caption{Model card information shown during onboarding.}
\end{figure}

\begin{figure}[h]
\centering
\resizebox{\textwidth}{!}{
\includegraphics{sc_study_bdd/sc7.PNG}
}
\caption{Prediction with AI interface (AI predicts no traffic light)}
\end{figure}

\begin{figure}[h]
\centering
\resizebox{\textwidth}{!}{
\includegraphics{sc_study_bdd/sc8.PNG}
}
\caption{Feedback shown during onboarding phase after human predicts.}
\end{figure}

\begin{figure}[h]
\centering
\resizebox{\textwidth}{!}{
\includegraphics{sc_study_bdd/sc9.PNG}
}
\caption{Feedback shown during onboarding phase after human predicts (sets of examples from region) }
\end{figure}

\begin{figure}[h]
\centering
\resizebox{\textwidth}{!}{
\includegraphics{sc_study_bdd/sc10.PNG}
}
\caption{Prediction with AI interface (AI predicts there is  a traffic light)}
\end{figure}

\begin{figure}[h]
\centering
\resizebox{\textwidth}{!}{
\includegraphics{sc_study_bdd/sc11.PNG}
}
\caption{Feedback shown during onboarding phase after human predicts (correct feedback)}
\end{figure}

\begin{figure}[h]
\centering
\resizebox{\textwidth}{!}{
\includegraphics{sc_study_bdd/sc12.PNG}
}
\caption{Testing phase instructions}
\end{figure}

\begin{figure}[h]
\centering
\resizebox{\textwidth}{!}{
\includegraphics{sc_study_bdd/sc13.PNG}
}
\caption{Testing phase instructions that include AI-integration recommendation}
\end{figure}

\begin{figure}[h]
\centering
\resizebox{\textwidth}{!}{
\includegraphics{sc_study_bdd/sc14.PNG}
}
\caption{Prediction interface with AI and with AI-integration recommendations.}
\end{figure}



==> todo.tex <==
algorithm box typo

list the hyperparameters clearly

learning rate and number of epochs

figure 3: step 2 annotate

table 5 order of columns 

table 2 cateogry


mmlu topics

dennis comments

conclusion section
